Jedi: Entropy-based Localization and Removal of Adversarial Patches

Real-world adversarial physical patches were shown to be successful in compromising state-of-the-art models in a variety of computer vision applications. Existing defenses that are based on either input gradient or features analysis have been compromised by recent GAN-based attacks that generate naturalistic patches. In this paper, we propose Jedi, a new defense against adversarial patches that is resilient to realistic patch attacks. Jedi tackles the patch localization problem from an information theory perspective; leverages two new ideas: (1) it improves the identification of potential patch regions using entropy analysis: we show that the entropy of adversarial patches is high, even in naturalistic patches; and (2) it improves the localization of adversarial patches, using an autoencoder that is able to complete patch regions from high entropy kernels. Jedi achieves high-precision adversarial patch localization, which we show is critical to successfully repair the images. Since Jedi relies on an input entropy analysis, it is model-agnostic, and can be applied on pre-trained off-the-shelf models without changes to the training or inference of the protected models. Jedi detects on average 90% of adversarial patches across different benchmarks and recovers up to 94% of successful patch attacks (Compared to 75% and 65% for LGS and Jujutsu, respectively).

==> sections/Conclusion.tex <==
In this paper, we present Jedi, a novel adversarial patch defense that leverages the higher entropy value of adversarial patches relative to natural image data to efficiently localize the adversarial patches and suppress them using inpainting. We also introduce an autoencoder step to further enhance the patch localization process. Our experimental results show that our method locates a large percentage of adversarial patches with a high detection quality and mitigates most successful attacks. These results generalize across many datasets, adversarial patch attacks and in both classification and detection tasks. Most notably, our method has shown its effectiveness against a recent adversarial patch generation method that claims to generate naturalistic patches. Furthermore, we demonstrate that our method is resistant to adaptive attacks: we have attempted to create low entropy patches in order to bypass our proposed defense. However, imposing an entropy restriction on the patch generation process results in patches that do not possess adversarial power. Jedi advances the state-of-the-art by highlighting the promising utility of entropy in the quest of robust machine learning. While this work is empirical, we will investigate a more theoretical perspective towards provably robust entropy-based defense. 
%although there are still some blind spots that should be considered in future adversarial patch defense work, namely attack patterns that apply multiple patches and multi-view detection scenarios.

==> sections/Related.tex <==
As CNNs are on the forefront of machine leaning research, it is no surprise that understanding the vulnerabilities of these CNNs and researching solutions to these issues is a very active field of research. As adversarial attacks and especially adversarial patches prove to be a threat to CNN based computer vision tasks, there is a rising need for methods to detect and mitigate such attacks.
In this section, we showcase the evolution of adversarial patch defenses: The first subsection discusses empirical adversarial patch defenses, while the second subsection focuses on certified patch defenses.

% \subsection{Adversarial patch attacks \ihsen{This is not related work--}}

% Adversarial attacks on CNNs have been proven possible by Biggio et al. \cite{biggio}, and Szegedy et al. \cite{szegedy_noise} proposed a method to generate an adversarial noise that when added to an input image, was able to fool classifiers. Numerous attacks have been proposed using the same approach of adding a nearly imperceptible noise to the input image, such as the Fast Gradient Sign Method \cite{FGSM}, Basic iterative Method \cite{BIM}, Carlini and Wagner attacks \cite{cw}, DeepFool \cite{deepfool}, One-pixel attacks \cite{onepixel} and more. 

% These threats were demonstrated to be of concern by Kurakin et al. \cite{BIM} by printing adversarial samples on paper and showing that they can still fool classifiers even through the lens of a mobile phone. Etimov et al. \cite{evt_stop} have studied this attack concept further by managing to fool road sign detectors using printed disturbed stop sign stickers placed on to of the original sticker. Eykholt et al. \cite{eot} propose an 'Expectation Over Transformation' framework in order to expand the scope of these attacks to a noise that can be added to an arbitrary 3D object, vastly increasing the adversarial noise's effectiveness in different unfavorable conditions such as different view angles. 
 
% A further development of adversarial attacks is the adversarial patch: Instead of attacking the whole image with adversarial noise, the attack is restricted to a limited area, but in exchange, the amplitude constraint is removed. The main advantage of these attacks is in the simplicity of their real life implementation: These attacks can easily be printed in a "patch" form and attached to any surface in view of the targeted detector's camera. Furthermore, these patches are universal: they are not specific to a certain input image or class, but can fool a classifier no matter the type of input image used. 

% The first "Adversarial Patch" was proposed by Brown et al \cite{advpatch}, where the authors mask a part of the image and replace it with adversarial noise to fool classifier towards the targeted wrong class. The authors use a modified variant of the Expectation Over Transformation variant framework to apply rotation and scaling operations to the patch. The patch is trained using a set of images and uses gradient descent as its optimizer.

% Karmon et al. \cite{lavan} introduce their LAVAN patch, in which they attempt to reduce the surface of the patch while keeping its success rates high. The authors show that even a patch that only occupies 2\% of the image area can be an effective attack. Furthermore, the authors avoid covering the main object in the input image by placing the patch in a  non-salient part of the image. The patch is optimized by maximizing the classifier's loss with regards to the correct class, thus ensuring that the output result is not correct, and by minimizing the loss with regards to the targeted class.

% Thys et al. \cite{yolopatch} target the YOLO family of object detectors by creating a patch that can be used to hide people from CNN-based person detectors. This patch is created using an Adam optimizer whose objective is to minimize a loss function composed of a sum three weighted sub-goal loss functions: First, a non-printability score to ensure that the patch can be easily printed. Second, a total variation score to ensure a smooth patch. And finally, the objectness score of the person to hide in order to be undetected.

% DPatch \cite{dpatch} targets object detectors in two different ways: It can target Region Proposal Networks by focusing all of the regions of interest toards the patch, therefore the RPN will not output the location of the object to detect. Also, the patch can attack image classification by maximizing the loss with regards to the correct class in the case of an untargeted attack, or by minimizing the loss towards the targeted class otherwise.

% To generate patches that do not cause suspicion, especially by humans who can easily notice computer-generated patches, Hu et al. \cite{naturalistic} propose their Naturalistic Patch, that attempts to emulate the appearance of a natural image. To do so, the authors combine Generative Adversarial Networks with adversarial gradients into a network that can generate adversarial patches that are inconspicuous when found in commonly seen objects while keeping high attack performance. The authors also augment their patch with transformations such as scaling, rotations, blurring or occlusions.

% Adversarial attacks and patches have evolved to be a very serious threat to be considered when deploying CNN based object detectors and classifiers especially in safety-critical applications. This evolution was spurred by the the need to make the implementation of these attacks simpler in real-life conditions while widening the scope of these attacks to be universal to all input images. Another factor of this evolution is the development of countermeasures to these attacks that may counteract their effects. These defenses are discussed in the next subsection.

%\subsection{Adversarial patch defenses}



\subsection{Empirical patch defenses}

This category of adversarial patch defenses attempts to leverage certain proprieties of adversarial patches that distinguish them from benign image inputs in order to warn to the presence of adversarial inputs and/or mitigate the attack to restore the original correct result. Such different proprieties can be found in pixel-level differences in the input images or in suspicious behavior in the features calculated by the CNN's layers. 

Naseer et al.\cite{lgs} propose their Local Gradient Smoothing defense, where they note that adversarial inputs have a higher frequency of pixel value changes around the patch location compared to benign samples. To find such areas, the authors calculate local image gradients using a sliding window and any windows where the gradient exceeds a certain threshold is kept in a gradient map. Finally, the gradient map is back-projected on the input image to suppress high frequency noise.

Hayes \cite{dw} introduces the Digital Watermarking defense, that leverages the tendency of adversarial patches to generate saliency maps that contain dense clusters around the patch. First, a saliency map is created with regards to the initial output class. This map is binarized according to a certain threshold in order to highlight cluster, and morphological operators are used to improve the quality of the map. Finally, this map is used as a mask for the inpainting operation to delete the suspected patch.

The LanCe adversarial patch defense by Xu et al. \cite{lance} uses irregular neuron activation patterns caused by the semantic inconsistency in adversarial patches to identify and suppress these patches. After the initial classification, a visual neuron activation map is generated and the image data around the area with the highest activation value is cropped. In parallel, a synthetic image of the originally detected class is generated and compared to the image crop obtained earlier in the frequency domain using a Jaccard Similarity metric. If the images are similar, the input is considered benign. Otherwise, the high activation area is considered an adversarial patch and inpainting is used to suppress the patch.

The adversarial patch defense proposed by Co et al. \cite{detect_uap}, also leverages the irregular neuron activation patterns to detect adversarial inputs. The authors avoid using the raw feature data as it can require large amount of memory especially in larger models. Instead, the mean and standard deviation of neuron activations are collected at a layer of the CNN and compared to a baseline level of activations from a known-clean sample of images. If there is a significant discrepancy, the input image is flagged as adversarial.

Chen et al. \cite{jujutsu} locate adversarial patches by utilizing their tendency to be the most salient object in the image. The first step is to determine whether the input image contains a patch. To do so, a saliency map is generated and a sliding window averaging operation is used to determine the area with the highest saliency. This area is then transplanted to a known-clean holdout image, and if the classification result of the holdout image changes to the result class of the input image, this area is determined to be an adversarial patch. If the presence of the patch is confirmed, the next step is to mitigate its presence by masking the area with high saliency and using inpainting to fill in the mask.

\subsection{Certified patch defenses}

While empirical patch defenses have shown promising performance, there is still an intense cat and mouse scenario where better attacks are constantly published that defeat these defenses. To avoid these situations, another category of adversarial patch defenses is certified defenses. Unlike empirical defenses, these defenses attempt to create neural networks whose goal is to "certify" that the result is provably robust for a given input and patch size. 

Levine and Feizi \cite{derandomized} propose their Derandomized Smoothing method for certified patch defense in which a "smoothed" classifier is created by using structured ablation on certain parts of the input image in order to mitigate patch attacks. This structured ablation can be in the form of blocks or bands, where pixels from outside the selected shape are removed. The final classification result is the class that was returned by the most ablations. The authors prove that their defense can be certified since only a minority of the set of ablations used is affected by the adversarial patch.

In the Patchguard certified defense \cite{patchguard}, the authors assert that adversarial patches are effective due to two reasons: First, the convolution operations pool information from a large area of the image, therefore giving the patch increased influence. Second, adversarial patches generate excessive feature values that point towards the wrong classification class. To remedy these issues, the authors propose to adopt CNN architectures that have smaller reception fields and to clip excessive feature values and check if the classification result changes to detect adversarial inputs.

Xiang et al. \cite{patchguardpp} further improve on their previous defense in Patchguard++: By adopting the same architectures proposed in Patchguard and adding a sliding window mask to the final feature map, the authors can detect adversarial patches by checking for changes in the output class that have a high confidence score. A similar approach was proposed at image level in the Minority Reports defense \cite{mr}, but it was deemed computationally infeasible when scaled for larger images. However, this method is possible in feature space as the inference step does not need to be repeated each time the window is moved. 

While adversarial patch defenses have shown significant progress over the last few years, there is still a long path ahead before current CNNs can be declared robust: Empirical defenses may have good performance against existing patch attacks, however they remain vulnerable to adaptive attacks. And while certified defenses can prove that some inputs under certain conditions may be impervious to all kinds of patch attacks, these defenses do not cover the whole spectrum of CNN applications and have not scaled up to today's large network and input sizes. Furthermore, patch attacks are rapidly becoming more effective and stealthy, which may render current defenses obsolete quickly. 


==> sections/Threat.tex <==
%\ihsen{Here we introduce our assumoptions, the objective of the attacker, the attack method, the knwoledge of the defender etc. }

\noindent\textbf{Attacker knowledge.} Our threat model assumes the attacker's objective is to create a universal adversarial patch. To do so, we presume that the attacker has a white-box access, with full knowledge of the targeted neural network network including the architecture, parameters and gradient. Moreover, we assume that the attacker has access to images  from the same distribution of the target system to generate the patch. The adversarial patches can be placed anywhere in the input image for the classification tasks, and the patches can be overlaid on the objects of interest for the detection tasks.

\noindent\textbf{Defender knowledge.} For the defending side, we assume that the defender has a set of known clean images to establish the entropy distribution of clean images, and that the defenders can create a set of masks to use as training data for the autoencoder. Although the last assumption can be waived if the defender uses our alternate method described in appendix A, at a small cost in performance.

% attacker:
% \begin{itemize}
%     \item objective : create a universal adversarial patch
%     \item white box scenario: has full access to the CNN, its structure and its weights
%     \item may have access to the input images we defend, or only a set of "similar" images, we study both scenarios anyways 
%     \item can replace any contiguous part of the image with a patch in classification tasks
%     \item can directly overlay the patch on the object of interest in detection tasks
% \end{itemize}

% defender:
% \begin{itemize}
%     \item has access to a known clean set of images from the to create the entropy statistical distribution
%     \item is able to create a set of masks of potential adversarial patch locations to train the autoencoder
%     \item (although the appendix shows that our method is feasible without an autoencoder at a cost in performance)
% \end{itemize}

